Intelligo ut Confido: Understanding, Trust and User Experience in Verifiable Receipt-Free E-Voting (long version)

Voting protocols seek to provide integrity and vote privacy in elections. To achieve integrity, procedures have been proposed allowing voters to verify their vote - however this impacts both the user experience and privacy. Especially, vote verification can lead to vote-buying or coercion, if an attacker can obtain documentation, i.e. a receipt, of the cast vote. Thus, some voting protocols go further and provide mechanisms to prevent such receipts. To be effective, this so-called receipt-freeness depends on voters being able to understand and use these mechanisms. In this paper, we present a study with 300 participants which aims to evaluate the voters' experience of the receipt-freeness procedures in the e-voting protocol Selene in the context of vote-buying. This actually constitutes the first user study dealing with vote-buying in e-voting. While the usability and trust factors were rated low in the experiments, we found a positive correlation between trust and understanding.

==> sections/exam_ryan.tex <==
\section{Advanced Protocols}


\noindent \textbf{Q1: Authenticated Key Exchange} 

Consider a case in which two honest parties Alice and Bob want to run a key exchange protocol over an insecure channel to establish a fresh high-entropy session key, but only share a low-entropy secret $pw$ (i.e. short password). We assume that Alice’s and Bob’s identity strings 'Alice' and 'Bob' are public (known to everyone including adversaries). Before engaging in a key exchange protocol, both Alice and Bob encode shared password $pw$ as a symmetric 256-bit key $spw$ by hashing $pw$ with $sha256$ hash function as follows: $spw = sha256(pw)$; Now, $spw$ can be used as an input key to a secure symmetric encryption algorithm $Enc_{spw}(message)$ that provides both confidentiality and integrity of the message. Look at the following two possible key exchange protocols:\\

\noindent \textbf{Protocol PWKE1:} Alice samples a random 256-bit secret $sk$ and creates a message to be encrypted by concatenating secret $sk$ to Alice’s and Bob’s identities as follows: $('Alice' \ || \ 'Bob' \ || \ sk)$; Next, Alice encrypts prepared message using $spw$ (derived from the shared password)
$$c = Enc_{spw}('Alice' \ || \ 'Bob' \ || \ sk)$$
and sends the obtained ciphertext $c$ to Bob. Upon receiving $c$, Bob decrypts it using $spw$, parses obtained plaintext, and checks whether the identities are valid. If all checks are fine, Bob saves $sk$ as a high-entropy secret shared with Alice.\\
\[
A \rightarrow B: c = Enc_{spw}('Alice' \ || \ 'Bob' \ || \ sk)
\]

\noindent \textbf{Protocol PWKE2:} In this alternative key exchange protocol, Alice and Bob use symmetric key $spw$ (derived from the shared password) to authenticate Diffie-Hellman Key Exchange (DHKE). PKWE2 goes as follows: Alice picks a random $x$, computes her DH key share $X = g^x$, creates a message by concatenating identities to $X$ value, encrypts it using $spw$ as $c_1 = Enc_{spw}('Alice' \ || \ 'Bob' \ || \ X)$, and sends the obtained ciphertext $c_1$ to Bob. Upon receiving $c_1$, Bob decrypts $c_1$ using $spw$, parses the obtained plaintext, and checks whether the identities are as expected. If all checks are fine, Bob saves $X$. Next, Bob picks a random $y$, computes his DH key share $Y = g^y$, creates and encrypts a message using $spw$ as $c_2 = Enc_{spw}('Bob' \ || \ 'Alice' \ || \ Y \ || \ X)$, and sends $c_2$ to Alice. Subsequently, Bob computes $sk = X^y$ and saves it as a high-entropy secret shared with Alice. Upon receiving $c_2$, Alice decrypts it using $spw$, parses the obtained plaintext, and checks whether received values are as expected. If all checks are fine, Alice saves $Y$. Next, Alice computes $sk = Y^x$ and saves it as a high-entropy secret shared with Bob.\\

\[
A \rightarrow B: c_1 = Enc_{spw}('Alice' \ || \ 'Bob' \ || \ X) \ \ \ \ \ 
\]
\[
B \rightarrow A: c_2 = Enc_{spw}('Bob' \ || \ 'Alice' \ || \ Y \ || \ X)
\]
\noindent \textbf{Questions:}
\begin{enumerate}
    \item What type of key exchange are the protocols: PWKE1 and PWKE2? (key agreement vs key transport) Briefly explain. (0.5 points)
    \item If an eavesdropping adversary Eve obtains the transcript $t = (c)$ of a single PWKE1 execution between Alice and Bob, can she somehow compute the corresponding session key? Explain why this is possible (or not). (1 points)
    \item If an eavesdropping adversary Eve obtains the transcript t = (c1, c2) of a single PWKE2 execution between Alice and Bob, can she somehow compute the corresponding session key sk? Explain why this is possible (or not). (1 points)
    \item If the password shared between Alice and Bob is compromised in some way (e.g. malware attack) and known to an active adversary, can such adversary impersonate Alice to Bob and vice versa in PWKE1? What about the same scenario in PWKE2? Explain. (1 point)
\end{enumerate}


\noindent \textbf{Q2: Verifiable Voting protocols-Ballot Assurance} 

Many end-to-end verifiable voting schemes involve the generation of an encryption of the voter's choice(s). We do not want to have to trust the device or entity creating these encryptions, but we want the voters to be confident that their vote is correctly encrypted. Describe a technique by which the voter can be assured that their vote is correctly represented in the ballot but without undermining receipt-freeness, i.e. without providing the voter with a way to convince a third party of the contents of the ballot. (1.5 point)

